Global Structure Knowledge-Guided Relation Extraction Method for Visually-Rich Document

Visual Relation Extraction (VRE) is a powerful means of discovering relationships between entities within visually-rich documents. Existing methods often focus on manipulating entity features to find pairwise relations, yet neglect the more fundamental structural information that links disparate entity pairs together. The absence of global structure information may make the model struggle to learn long-range relations and easily predict conflicted results. To alleviate such limitations, we propose a GlObal Structure knowledge-guided relation Extraction (GOSE) framework. GOSE initiates by generating preliminary relation predictions on entity pairs extracted from a scanned image of the document. Subsequently, global structural knowledge is captured from the preceding iterative predictions, which are then incorporated into the representations of the entities. This "generate-capture-incorporate" cycle is repeated multiple times, allowing entity representations and global structure knowledge to be mutually reinforced. Extensive experiments validate that GOSE not only outperforms existing methods in the standard fine-tuning setting but also reveals superior cross-lingual learning capabilities; indeed, even yields stronger data-efficient performance in the low-resource setting. The code for GOSE will be available at https://github.com/chenxn2020/GOSE.

==> Tables/all_experiment.tex <==
\begin{table*}[htbp!]
\centering
\scalebox{0.70}{
\begin{tabular}{@{}clccccccccc@{}}
\toprule
% 标准fine-tune
\multicolumn{1}{c}{\multirow{2}{*}{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{Model}} &FUNSD & \multicolumn{7}{c}{XFUND}         & \multirow{2}{*}{Avg.} \\ \cmidrule(l){3-3}  \cmidrule(l){4-10} &                                  & EN    & ZH & JA & ES & FR & IT & DE & PT &                      \\ \midrule \midrule

\multirow{8}{*}{Language-specific fine-tuning}  & XLM-RoBERTa$_{\mathrm{BASE}}$            &  0.2659 &  0.5105  & 0.5800  & 0.5295 &  0.4965  & 0.5305 &  0.5041 &  0.3982  & 0.4769  \\
& InfoXLM$_{\mathrm{BASE}}$               &  0.2920 &  0.5214  & 0.6000  & 0.5516 &  0.4913  & 0.5281 &  0.5262  & 0.4170  & 0.4910    \\
& LayoutXLM$_{\mathrm{BASE}}$                  &  0.5483  & 0.7073  & 0.6963 &  0.6896 &  0.6353  & 0.6415 &  0.6551 &  0.5718  & 0.6432 \\

&LayoutXLM+CPE&&&&&&&&& \\
&XYLayoutLM$_{\mathrm{BASE}}$&&&&&&&&& \\

& \textbf{LiLT[}InfoXLM\textbf{]}$_{\mathrm{BASE}}$                   &  \textbf{0.6276 }                     &   \textbf{0.7297   }               &     \textbf{0.7037   }             &        \textbf{0.7195 }            &    \textbf{0.6965     }            &          \textbf{0.7043  }         &         \textbf{0.6558   }         &      \textbf{0.5874    }           &  \textbf{0.6781} \\

\cmidrule(l){2-11}
&Ours&&&&&&&&& \\
&Ours&&&&&&&&& \\
\midrule  \midrule

% 跨语言迁移
\multirow{6}{*}{Cross-lingual zero-shot transfer}  & XLM-RoBERTa$_{\mathrm{BASE}}$                   &  0.2659 &0.1601& 0.2611 &0.2440 &0.2240 &0.2374 &0.2288 &0.1996& 0.2276 \\
& InfoXLM$_{\mathrm{BASE}}$                     &  0.2920& 0.2405 &0.2851 &0.2481 &0.2454& 0.2193 &0.2027 &0.2049 &0.2423  \\
& LayoutXLM$_{\mathrm{BASE}}$                 &  0.5483& 0.4494& 0.4408 &0.4708 &0.4416 &0.4090 &0.3820& 0.3685 &0.4388  \\
& \textbf{LiLT[}InfoXLM\textbf{]}$_{\mathrm{BASE}}$                    &    \textbf{0.6276}                   &     \textbf{0.4764}               &    \textbf{0.5081}                 &     \textbf{0.4968}            & \textbf{0.5209}               &   \textbf{0.4697}             &   \textbf{0.4169  }              &  \textbf{0.4272 }         &  \textbf{0.4930 } \\

\cmidrule(l){2-11} 
&Ours&&&&&&&&& \\
&Ours&&&&&&&&& \\

\midrule  \midrule


% 多任务fine-tune
\multirow{6}{*}{Multitask fine-tuning}  
 & XLM-RoBERTa$_{\mathrm{BASE}}$                  &   0.3638 &  0.6797  & 0.6829 &  0.6828 &  0.6727  & 0.6937 &  0.6887  & 0.6082  & 0.6341                     \\
& InfoXLM$_{\mathrm{BASE}}$                      &    0.3699 &  0.6493  & 0.6473 &  0.6828 &  0.6831  & 0.6690 &  0.6384 &  0.5763 &  0.6145        \\
& LayoutXLM$_{\mathrm{BASE}}$                   &    0.6671 &  0.8241 &  0.8142 &  0.8104 &  0.8221  & 0.8310 &  0.7854  & 0.7044 &  0.7823      \\
& \textbf{LiLT[}InfoXLM\textbf{]}$_{\mathrm{BASE}}$                 &   \textbf{ 0.7407   }                   &       \textbf{ 0.8471  }            &     \textbf{0.8345  }               &     \textbf{  0.8335   }            &  \textbf{  0.8466   }               &       \textbf{ 0.8458       }       &     \textbf{  0.7878     }          &  \textbf{0.7643    }               &   \textbf{0.8125   } \\

\cmidrule(l){2-11} 
&Ours&&&&&&&&& \\
&Ours&&&&&&&&& \\

\bottomrule 

\end{tabular}}
\caption{Language-specific fine-tuning F1 accuracy on FUNSD and XFUND (fine-tuning on X, testing on X). “SER” denotes the semantic entity recognition and “RE” denotes the relation extraction.  \textbf{[]} indicates the off-the-shelf textual model used as the text flow of LiLT.}
\label{tab:language-specific}
\end{table*}

==> Tables/few.tex <==
\begin{table}[!tb]
     
 
    % \small
    % \footnotesize
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c | c | c | c | c | c}
        \toprule

        \textbf{Dataset} & \textbf{Model} 
        & \textbf{$K = 8$}  & \textbf{$K = 16$} & \textbf{$K = 32$} & \textbf{$K = 64$} \\
                \midrule
        

        \multirow{4}*{FUNSD} 
        & LayoutXLM$_{\mathrm{BASE}}$  & \cxn{TODO} & - & - & - \\
        & {\model}$_{LayoutXLM}$
        & -
        & - 
        & - 
        & -  \\
        
        & LiLT$_{\mathrm{BASE}}$ & 0.1250 & 0.2377 & 0.3722 & 0.4341 \\
        % \cmidrule(l){2-6}
        
        
        & {\model}$_{LiLT}$
        & \textbf{0.2102}   
        & \textbf{0.3260} 
        & \textbf{0.4763} 
        & \textbf{0.6146}  \\
        \bottomrule
        
    \end{tabular}}
    \caption{
    Results of compared models for VRE on the few-shot setting.
     We report the results of F1 accuracy and adopt $K =8, 16, 32, 64$ (\# training samples).}
    \label{tab:few}
\end{table}
